Bloch-Beilinson conjectures for Hecke characters and Eisenstein cohomology of Picard surfaces

We consider certain families of Hecke characters $\phi$ over a quadratic imaginary field $F$. According to the Bloch-Beilinson conjectures, the order of vanishing of the $L$-function $L(\phi,s)$ at the central point $s=-1$ should be equal to the dimension of the space of extensions of the Tate motive $\mathbb{Q}(1)$ by the motive associated with $\phi$. In this article, we construct candidates for the corresponding extensions of Hodge structures, assuming that the sign of the functional equation of $L(\phi,s)$ is $-1$. This is accomplished through the cohomology of variations of Hodge structures over Picard modular surfaces associated with $F$ and Harder's theory of Eisenstein cohomology. Furthermore, we demonstrate that these extensions are naturally realized within certain biextensions. We outline a program to compute the biextension height and utilize it to establish the non-triviality of these extensions.

==> macros.tex <==
\usepackage[a4paper,centering,left=3.4cm,right=3.4cm]{geometry}
\usepackage{amsfonts,amscd,amssymb,amsmath,amsthm,mathrsfs,multirow,xcolor,lscape}
\usepackage{longtable,pbox,lipsum, stmaryrd,url, epstopdf, float, enumerate}
\usepackage[all,cmtip]{xy}
\usepackage[english]{babel}
\usepackage{color}

\usepackage{ucs}
\usepackage[utf8]{inputenc}
\usepackage{dsfont}
\usepackage[T1]{fontenc} 
\usepackage{lmodern}
\usepackage[thinlines]{easytable}

\usepackage{phaistos}
\usepackage{microtype}

\usepackage{enumitem}
\setcounter{tocdepth}{1}

\usepackage{scalerel}
\usepackage{todonotes}
\usepackage{stackengine,wasysym}
\usepackage{todonotes}
\usepackage[T1]{fontenc}

\usepackage[colorlinks,linkcolor=blue,anchorcolor=blue,citecolor=blue,backref=page]{hyperref}
\usepackage{hyperref}

\def\test#1{$%
  \reallywidetilde{#1}\,
  \scriptstyle\reallywidetilde{#1}\,
  \scriptscriptstyle\reallywidetilde{#1}
$\par}

%----------------------------------------------------------------------------------------
%	THEOREM STYLES
%----------------------------------------------------------------------------------------


\newtheorem{thm}{Theorem}[section]
\newtheorem{thmi}{Theorem}
\newtheorem{defi}[thm]{Definition}
\newtheorem{lemma}[thm]{Lemma}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{coro}[thm]{Corollary}
\newtheorem{rmk}[thm]{Remark}
\newtheorem{conjecture}[thm]{Conjecture}
\newtheorem{conjecture*}{Conjecture}
\newtheorem{notation}[thm]{Notation}
\newtheorem{convention}[thm]{Convention}
\newtheorem{obs}[thm]{Observation}
\newtheorem{pro}[thm]{Property}
\newtheorem*{theorem*}{Main Theorem}

%------------------- Tikz library ----------------------------%

%\setcounter{tocdepth}{1} 
\usepackage[all,cmtip]{xy}
\usepackage{tikz}
\usetikzlibrary{arrows} 
\usetikzlibrary{matrix}
\usetikzlibrary{calc}

%--------------- Tikz Library ends here ---------------------------%

%----------- Put the comment sign  before everything above---------%
%---------------------------------------------------------------------------------%
%               MACROS                                      
%---------------------------------------------------------------------------------%
\newcommand\scalemath[2]{\scalebox{#1}{\mbox{\ensuremath{\displaystyle #2}}}}

\newcommand{\T}{\mathrm{T}}

\newcommand{\m}{\mathcal{M}}

\newcommand{\rB}{\mathrm{B}}
\newcommand{\rG}{\mathrm{G}}
\newcommand{\rK}{\mathrm{K}}
\newcommand{\rP}{\mathrm{P}}
\newcommand{\ri}{\mathrm{i}}
\newcommand{\rL}{\mathrm{L}}
\newcommand{\rM}{\mathrm{M}}
\newcommand{\rN}{\mathrm{N}}
\newcommand{\rS}{\mathrm{S}}
\newcommand{\rT}{\mathrm{T}}
\newcommand{\rZ}{\mathrm{Z}}

\newcommand{\eqr}[1]{\mbox{(\ref{eq:#1})}}
%\newcommand{\ie}{i.e.\ }
\newcommand{\mr}[1]{\mathrm{#1}}

\newcommand{\tm}{\widetilde{\m}}


\newcommand{\BA}{{\mathbb{A}}}
\newcommand{\BB}{{\mathbb{B}}}
\newcommand{\BC}{{\mathbb{C}}}
\newcommand{\BD}{{\mathbb{D}}}
\newcommand{\BE}{{\mathbb{E}}}
\newcommand{\BF}{{\mathbb{F}}}
\newcommand{\BG}{{\mathbb{G}}}
\newcommand{\BH}{{\mathbb{H}}}
\newcommand{\BI}{{\mathbb{I}}}
\newcommand{\BJ}{{\mathbb{J}}}
\newcommand{\BK}{{\mathbb{K}}}
\newcommand{\BL}{{\mathbb{L}}}
\newcommand{\BM}{{\mathbb{M}}}
\newcommand{\BN}{{\mathbb{N}}}
\newcommand{\BO}{{\mathbb{O}}}
\newcommand{\BP}{{\mathbb{P}}}
\newcommand{\BQ}{{\mathbb{Q}}}
\newcommand{\BR}{{\mathbb{R}}}
\newcommand{\BS}{{\mathbb{S}}}
\newcommand{\BT}{{\mathbb{T}}}
\newcommand{\BU}{{\mathbb{U}}}
\newcommand{\BV}{{\mathbb{V}}}
\newcommand{\BW}{{\mathbb{W}}}
\newcommand{\BX}{{\mathbb{X}}}
\newcommand{\BY}{{\mathbb{Y}}}
\newcommand{\BZ}{{\mathbb{Z}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\Fa}{{\mathfrak{a}}}
\newcommand{\Fb}{{\mathfrak{b}}}
\newcommand{\Fc}{{\mathfrak{c}}}
\newcommand{\Fd}{{\mathfrak{d}}}
\newcommand{\Fe}{{\mathfrak{e}}}
\newcommand{\Ff}{{\mathfrak{f}}}
\newcommand{\Fg}{{\mathfrak{g}}}
\newcommand{\Fh}{{\mathfrak{h}}}
\newcommand{\Fi}{{\mathfrak{i}}}
\newcommand{\Fj}{{\mathfrak{j}}}
\newcommand{\Fk}{{\mathfrak{k}}}
\newcommand{\Fl}{{\mathfrak{l}}}
\newcommand{\Fm}{{\mathfrak{m}}}
\newcommand{\Fn}{{\mathfrak{n}}}
\newcommand{\Fo}{{\mathfrak{o}}}
\newcommand{\Fp}{{\mathfrak{p}}}
\newcommand{\Fq}{{\mathfrak{q}}}
\newcommand{\Fr}{{\mathfrak{r}}}
\newcommand{\Fs}{{\mathfrak{s}}}
\newcommand{\Ft}{{\mathfrak{t}}}
\newcommand{\Fu}{{\mathfrak{u}}}
\newcommand{\Fv}{{\mathfrak{v}}}
\newcommand{\Fw}{{\mathfrak{w}}}
\newcommand{\Fx}{{\mathfrak{x}}}
\newcommand{\Fy}{{\mathfrak{y}}}
\newcommand{\Fz}{{\mathfrak{z}}}

\newcommand{\FA}{{\mathfrak{A}}}
\newcommand{\FB}{{\mathfrak{B}}}
\newcommand{\FC}{{\mathfrak{C}}}
\newcommand{\FD}{{\mathfrak{D}}}
\newcommand{\FE}{{\mathfrak{E}}}
\newcommand{\FF}{{\mathfrak{F}}}
\newcommand{\FG}{{\mathfrak{G}}}
\newcommand{\FH}{{\mathfrak{H}}}
\newcommand{\FI}{{\mathfrak{I}}}
\newcommand{\FJ}{{\mathfrak{J}}}
\newcommand{\FK}{{\mathfrak{K}}}
\newcommand{\FL}{{\mathfrak{L}}}
\newcommand{\FM}{{\mathfrak{M}}}
\newcommand{\FN}{{\mathfrak{N}}}
\newcommand{\FO}{{\mathfrak{O}}}
\newcommand{\FP}{{\mathfrak{P}}}
\newcommand{\FQ}{{\mathfrak{Q}}}
\newcommand{\FR}{{\mathfrak{R}}}
\newcommand{\FS}{{\mathfrak{S}}}
\newcommand{\FT}{{\mathfrak{T}}}
\newcommand{\FU}{{\mathfrak{U}}}
\newcommand{\FV}{{\mathfrak{V}}}
\newcommand{\FW}{{\mathfrak{W}}}
\newcommand{\FX}{{\mathfrak{X}}}
\newcommand{\FY}{{\mathfrak{Y}}}
\newcommand{\FZ}{{\mathfrak{Z}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\CA}{{\cal A}}
\newcommand{\CB}{{\mathcal B}}
\newcommand{\CC}{{\cal C}}

\newcommand{\CE}{{\cal E}}
\newcommand{\CF}{{\cal F}}
\newcommand{\CG}{{\cal G}}

\newcommand{\CI}{{\cal I}}
\newcommand{\CJ}{{\cal J}}
\newcommand{\CK}{{\cal K}}
\newcommand{\CL}{{\cal L}}
\newcommand{\CM}{{\cal M}}
\newcommand{\CN}{{\mathcal N}}
\newcommand{\CO}{{\cal O}}
\newcommand{\CP}{{\cal P}}
\newcommand{\CQ}{{\cal Q}}
\newcommand{\CR}{{\cal R}}
\newcommand{\CS}{{\cal S}}
\newcommand{\CT}{{\cal T}}
\newcommand{\CU}{{\cal U}}
\newcommand{\CV}{{\cal V}}
\newcommand{\CW}{{\mathcal W}}
\newcommand{\CX}{{\cal X}}
\newcommand{\CY}{{\cal Y}}
\newcommand{\CZ}{{\cal Z}}

\newcommand{\cyrb}{{\cyr B}} 

\newcommand{\one}{\mathds{1}}

\newcommand{\omg}{\mathop{\rm \omega}\nolimits}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\End}{\mathop{\rm End}\nolimits}
\newcommand{\Hom}{\mathop{\rm Hom}\nolimits}
\newcommand{\Ext}{\mathop{\rm Ext}\nolimits}
\newcommand{\Sym}{\mathop{\rm Sym}\nolimits}
\newcommand{\Rep}{\mathop{\rm Rep}\nolimits}
\newcommand{\Res}{\mathop{\rm Res}\nolimits}
\newcommand{\Spec}{\mathop{\rm Spec}\nolimits}
\newcommand{\pt}{\boldsymbol{\cdot}}
\newcommand{\Gal}{\mathop{\rm Gal}\nolimits}
\newcommand{\CH}{\mathop{\rm CH}\nolimits}
\newcommand{\CHM}{\mathop{\rm CHM}\nolimits}
\newcommand{\DM}{\mathop{\rm DM}\nolimits}
\newcommand{\DBM}{\mathop{DM_{\text{\cyrb}}}\nolimits}
\newcommand{\DBcM}{\mathop{DM_{\text{\cyrb},c}}\nolimits}
\newcommand{\MM}{\mathop{\rm MM}\nolimits}
\newcommand{\NM}{\mathop{\rm NM}\nolimits}
\newcommand{\PL}{\mathop{\rm PL}\nolimits}
\newcommand{\Id}{\mathop{\rm Id}\nolimits}
\newcommand{\HS}{\mathop{\rm HS}\nolimits}
\newcommand{\MHS}{\mathop{\rm MHS}\nolimits}
\newcommand{\D}{\mathop{\rm D}\nolimits}
\newcommand{\SL}{\mathop{\rm SL} \nolimits}
\newcommand{\So}{\mathop{\rm SO} \nolimits}
\newcommand{\Sp}{\mathop{\rm Sp} \nolimits}
\newcommand{\GL}{\mathop{\rm GL} \nolimits}
\newcommand{\PGL}{\mathop{\rm PGL} \nolimits}
\newcommand{\Or}{\mathop{\rm O} \nolimits}
\newcommand{\POr}{\mathop{\rm PO} \nolimits}
\newcommand{\GSp}{\mathop{\rm GSp} \nolimits}
\newcommand{\U}{\mathop{\rm U} \nolimits}
\newcommand{\SU}{\mathop{\rm SU} \nolimits}
\newcommand{\GU}{\mathop{\rm GU} \nolimits}
\newcommand{\Ind}{\mathop{\rm Ind} \nolimits}
\newcommand{\IndUn}{\mathop{\rm IndUn} \nolimits}
\newcommand{\ind}{\mathop{\rm ind} \nolimits}
\newcommand{\Stab}{\mathop{\rm Stab} \nolimits}
\newcommand{\der}{\mathop{\rm \tiny{der}} \nolimits}
\newcommand{\ad}{\mathop{\rm \tiny{ad}} \nolimits}
\newcommand{\Gr}{\mathop{\rm Gr} \nolimits}
\newcommand{\im}{\mathop{\rm Im} \nolimits}
\newcommand{\can}{\mathop{\rm \tiny{can}} \nolimits}
\newcommand{\cusp}{\mathop{\rm \tiny{cusp}} \nolimits}
\newcommand{\et}{\mathop{\rm \tiny{ét}} \nolimits}
\newcommand{\op}{\mathop{\rm \tiny{op}} \nolimits}
\newcommand{\gal}{\mathop{\rm \tiny{gal}} \nolimits}
\newcommand{\num}{\mathop{\rm \tiny{num}} \nolimits}
\newcommand{\ord}{\mathop{\rm \tiny{ord}} \nolimits}
\newcommand{\diag}{\mathop{\rm diag} \nolimits}
\newcommand{\G}{\mathop{\tilde{\rm G}} \nolimits}
\newcommand{\Tr}{\mathop{\tilde{\rm T}} \nolimits}
\newcommand{\Un}{\mathop{\tilde{\rm U}} \nolimits}
\newcommand{\dm}{\mathop{\rm d} \nolimits}
\newcommand{\B}{\mathop{\tilde{\rm B}} \nolimits}
\newcommand{\K}{\mathop{\tilde{\rm K}_{\infty}} \nolimits}
\newcommand{\Ml}{\mathop{\tilde{\rm M}_{\lambda}} \nolimits}
\newcommand{\MlC}{\mathop{\tm_{\lambda, \BC}} \nolimits}
\newcommand{\Eis}{\mathop{\rm Eis} \nolimits}
\newcommand{\Ker}{\mathop{\rm Ker} \nolimits}
\newcommand{\Coker}{\mathop{\rm Coker} \nolimits}
\newcommand{\Img}{\mathop{\rm Im} \nolimits}
\newcommand{\dlt}{\mathop{\vert \delta \vert} \nolimits}
\newcommand{\dltv}{\mathop{\vert \delta_v \vert} \nolimits}
\newcommand{\loc}{\mathop{\rm loc} \nolimits}
\newcommand{\hc}{\mathop{\phi^{(1)}} \nolimits}
\newcommand{\hcq}{\mathop{\phi^{(1)}_{\BQ}} \nolimits}
\newcommand{\hol}{\mathop{\rm \tiny{hol}} \nolimits}
\newcommand{\topo}{\mathop{\rm \tiny{top}} \nolimits}

%\newcommand{\iu}{\mathop{\texttt{i}} \nolimits}

\newcommand{\iu}{\mathsf{i}}

\newcommand{\tmt}[4]{\left({#1\atop #3}{#2\atop #4}\right)}

\newcommand{\q}[1]{``#1''}
\newcommand\restr[2]{{% we make the whole thing an ordinary symbol
  \left.\kern-\nulldelimiterspace % automatically resize the bar with \right
  #1 % the function
  %\vphantom{\big|} % pretend it's a little taller at normal size
  \right|_{#2} % this is the delimiter
  }}



\newcommand{\dr}{\mathsf{d}r}
\newcommand{\dd}{\mathsf{d}}
\newcommand{\dl}{\mathsf{d}l}
\newcommand{\pp}{\mathsf{p}}
\newcommand{\ccc}{\mathsf{c}}
\newcommand{\ddd}{\mathsf{d}}
\newcommand{\ppp}{\mathsf{p}}
\newcommand{\qqq}{\mathsf{q}}



%----------------------------------------------------------------------------------------
%	OUR COMMANDS
%----------------------------------------------------------------------------------------

\newcommand{\jitendra}[1]{{\color{red} \sf $\heartsuit\heartsuit$ Jitendra: [#1]}}
\newcommand{\mattia}[1]{{\color{purple} \sf $\clubsuit\clubsuit$ Mattia: [#1]}}
\newcommand{\jb}[2][]{\todo[#1,color=red!20]{JB: #2}}
\newcommand{\mc}[2][]{\todo[#1,color=green!30]{MC: #2}}
%-----------------------------------------------------------------------------------------------


